FedNoisy: Federated Noisy Label Learning Benchmark

Federated learning has gained popularity for distributed learning without aggregating sensitive data from clients. But meanwhile, the distributed and isolated nature of data isolation may be complicated by data quality, making it more vulnerable to noisy labels. Many efforts exist to defend against the negative impacts of noisy labels in centralized or federated settings. However, there is a lack of a benchmark that comprehensively considers the impact of noisy labels in a wide variety of typical FL settings. In this work, we serve the first standardized benchmark that can help researchers fully explore potential federated noisy settings. Also, we conduct comprehensive experiments to explore the characteristics of these data settings and the comparison across baselines, which may guide method development in the future. We highlight the 20 basic settings for 6 datasets proposed in our benchmark and standardized simulation pipeline for federated noisy label learning, including implementations of 9 baselines. We hope this benchmark can facilitate idea verification in federated learning with noisy labels. \texttt{FedNoisy} is available at \codeword{https://github.com/SMILELab-FL/FedNoisy}.

==> subfile/6_conclude.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this paper, we propose comprehensive data settings and standardized simulation pipeline for FNLL in benchmark \texttt{FedNoisy}, including 20 basic data settings for potential FNLL settings, 5 datasets, and 8 baselines covering a wide scope of methodologies.
We conduct extensive comparisons and reveal some special characteristics of FNLL, which we hope can motivate further research on noisy label learning in FL community. Currently, \texttt{FedNoisy} is implemented on PyTorch \cite{NEURIPS2019_9015} and FedLab \cite{JMLR:v24:22-0440}, which might limit the usage of researchers familiar with other ML backends and FL frameworks, such as TensorFlow \cite{tensorflow2015-whitepaper}, Flower \cite{beutel2020flower}, FedML \cite{he2020fedml}. Supporting other backends/frameworks is one of the future directions. We will keep updating \texttt{FedNoisy} to support more datasets and FNLL baselines.

==> subfile/acknow.tex <==
\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2023/PaperInformation/FundingDisclosure}.
You can use the \texttt{ack} environment provided in the style file. As opposed to the main NeurIPS track, acknowledgements do not need to be hidden.
\end{ack}
